Pron vs Prompt: Can Large Language Models already Challenge a World-Class Fiction Author at Creative Text Writing?

It has become routine to report research results where Large Language Models (LLMs) outperform average humans in a wide range of language-related tasks, and creative text writing is no exception. It seems natural, then, to raise the bid: Are LLMs ready to compete in creative writing skills with a top (rather than average) novelist? To provide an initial answer for this question, we have carried out a contest between Patricio Pron (an awarded novelist, considered one of the best of his generation) and GPT-4 (one of the top performing LLMs), in the spirit of AI-human duels such as DeepBlue vs Kasparov and AlphaGo vs Lee Sidol. We asked Pron and GPT-4 to provide thirty titles each, and then to write short stories for both their titles and their opponent's. Then, we prepared an evaluation rubric inspired by Boden's definition of creativity, and we collected 5,400 manual assessments provided by literature critics and scholars. The results of our experimentation indicate that LLMs are still far from challenging a top human creative writer, and that reaching such level of autonomous creative writing skills probably cannot be reached simply with larger language models.

==> sections/X_acknowledgments.tex <==
\section*{Acknowledgments}

We would like to thank the literary experts and evaluators who participated in this study for their valuable insights and contributions. This work was supported by [Funding Information]

This work has been financed  by the European Union (NextGenerationEU funds) through the ``Plan de Recuperación, Transformación y Resiliencia'', by the Ministry of Economic Affairs and Digital Transformation and by the UNED University. Spanish government Ph.D. research grant ({\it Ministerio de Universidades}) FPU20/07321. However, the points of view and opinions expressed in this document are solely those of the author(s) and do not necessarily reflect those of the European Union or European Commission. Neither the  European Union nor the European Commission can be considered responsible for them. 
.

==> tables/rubric.tex <==
\begin{table*}[ht]
\centering
\caption{Evaluate the attractiveness of the following aspects of the text, understanding it as a literary object.}
\begin{tabularx}{\textwidth}{|X|X|X|}
\hline
\textbf{Aspect} & \textbf{Question} & \textbf{Options} \\
\hline
\textbf{Title} & Does the title seem attractive to you? Does it catch your attention and make you interested in the synopsis? & 0: It does not catch attention or generate any interest in the story. \newline
1: It barely catches attention but does elicit slight interest. \newline
2: It is suggestive and sparks curiosity. \newline
3: It is captivating and generates high expectations for the text. \\
\hline
\textbf{Style} & Does the style seem attractive and make you enjoy reading the synopsis? & 0: The style lacks attractiveness and even discourages reading. \newline
1: The style has slight attractiveness but does not particularly stand out. \newline
2: The style is attractive and contributes to the enjoyment of reading. \newline
3: The style is captivating in itself, creating a memorable reading experience. \\
\hline
\textbf{Story and Characters} & Do the story and characters seem attractive and capture your interest in the theme itself? & 0: The story and characters lack attractiveness, with no elements that stand out or add value. \newline
1: The story and characters have some attractiveness but lack elements that capture attention. \newline
2: The story and characters are quite attractive and capture attention. \newline
3: The story and characters are very attractive and completely capture attention. \\
\hline
\end{tabularx}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Evaluate the originality of the following aspects of the text. We understand that a text is original if it surprises you (if it is something you did not expect, if it is unfamiliar or reminds you of things you have read before) regardless of whether you found it attractive or not.}
\begin{tabularx}{\textwidth}{|X|X|X|}
\hline
\textbf{Aspect} & \textbf{Question} & \textbf{Options} \\
\hline
\textbf{Title} & Does the title seem original to you? & 0: The title is very predictable, a pure cliché. \newline
1: The title is quite predictable and resorts to clichés. \newline
2: The title is quite original and avoids clichés. \newline
3: The title is unique and surprising, unlike anything you have seen before. \\
\hline
\textbf{Style} & Is the text's style original and surprising? & 0: The style is formulaic and completely conventional. \newline
1: The style has some original elements but is predominantly conventional. \newline
2: The style is relatively original and is not easily comparable to other writers. \newline
3: The style is very original and reveals a unique voice of the writer. \\
\hline
\textbf{Plot} & Is the plot of the text original and introduces innovative elements? & 0: The plot is completely conventional and relies on widely explored ideas or clichés without bringing new elements. \newline
1: The plot is quite conventional, although there are marginal attempts to introduce original elements. \newline
2: The plot is quite original and brings innovative elements. \newline
3: The plot is very original and innovative. \\
\hline
\end{tabularx}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Considering that the title was the starting point of the literary exercise, do you think the writer knew how to use it well?}
\begin{tabularx}{\textwidth}{|X|X|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Considering that the title was the starting point of the literary exercise, do you think the writer has used it well? & No relation at all between the title and the synopsis. \newline
The relation between the title and the synopsis is almost irrelevant. \newline
There is some relation between the title and the synopsis, although not evident. \newline
There is a lot of relation between the title and the synopsis, and the text's development is predictable from the title. \newline
There is a lot of relation between the title and the synopsis, and the connection is surprising; the way of developing the title is original. \\
\hline
\end{tabularx}
\end{table*}

\begin{table*}[ht]
\centering
\caption{It values the creativity of:}
\begin{tabularx}{\textwidth}{|X|X|}
\hline
\textbf{Aspect} & \textbf{Options} \\
\hline
\textbf{Title} & 0: Not creative at all. \newline
1: Slightly creative. \newline
2: Quite creative. \newline
3: Very creative. \\
\hline
\textbf{Synopsis} & 0: Not creative at all. \newline
1: Slightly creative. \newline
2: Quite creative. \newline
3: Very creative. \\
\hline
\end{tabularx}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Do you think it is possible that the text was totally or partially written by:}
\begin{tabularx}{\textwidth}{|X|X|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Who do you think wrote this title? & A novel writer. \newline
An established writer. \newline
An artificial intelligence. \\
\hline
Who do you think wrote the synopsis? & A novel writer. \newline
An established writer. \newline
An artificial intelligence. \\
\hline
\end{tabularx}
\end{table*}

\begin{table*}[ht]
\centering
\caption{The exercise of inventing a synopsis for an imaginary movie can be seen as a sort of literary genre:}
\begin{tabularx}{\textwidth}{|X|X|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Do you think you would select this text for an anthology of this genre? & 0: Under no circumstances. \newline
1: It is unlikely. \newline
2: It is probable. \newline
3: With certainty. \\
\hline
Do you think your evaluation of the text would align with the majority of readers? & 0: Under no circumstances. \newline
1: It is unlikely. \newline
2: It is probable. \newline
3: With certainty. \\
\hline
Do you think your evaluation of the text would align with the majority of literary critics? & 0: Under no circumstances. \newline
1: It is unlikely. \newline
2: It is probable. \newline
3: With certainty. \\
\hline
Judging only by this text, do you think it is likely that the author has a recognizable style, that is, a unique voice? & 0: Under no circumstances. \newline
1: It is unlikely. \newline
2: It is probable. \newline
3: With certainty. \\
\hline
\end{tabularx}
\end{table*}



==> tables/rubric2.tex <==
\section*{1. Rate the attractiveness of the following aspects of the text, considering it as a literary object.}

\begin{longtable}{|p{0.2\textwidth}|p{0.5\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Aspect} & \textbf{Question} & \textbf{Options} \\
\hline
\textbf{Title} & Does the title seem attractive to you? Does it catch your attention and make you interested in the synopsis? & 
0 It does not catch attention or generate any interest in the story. \\
& & 1 It barely catches attention but does elicit slight interest. \\
& & 2 It is suggestive and sparks curiosity. \\
& & 3 It is captivating and generates high expectations for the text. \\
\hline
\textbf{Style} & Does the style seem attractive and make you enjoy reading the synopsis? & 
0 The style lacks attractiveness and even discourages reading. \\
& & 1 The style has slight attractiveness but does not particularly stand out. \\
& & 2 The style is attractive and contributes to the enjoyment of reading. \\
& & 3 The style is captivating in itself, creating a memorable reading experience. \\
\hline
\textbf{Story and Characters} & Do the story and characters seem attractive and capture your interest in the theme itself? & 
0 The story and characters lack attractiveness, with no elements that stand out or add value. \\
& & 1 The story and characters have some attractiveness but lack elements that capture attention. \\
& & 2 The story and characters are quite attractive and capture attention. \\
& & 3 The story and characters are very attractive and completely capture attention. \\
\hline
\end{longtable}

\section*{2. Rate the originality of the following aspects of the text. We understand that a text is original if it surprises you (if it is something unexpected, if it does not seem familiar or remind you of things you have read before) regardless of whether you found it attractive or not.}

\begin{longtable}{|p{0.2\textwidth}|p{0.5\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Aspect} & \textbf{Question} & \textbf{Options} \\
\hline
\textbf{Title} & Does the title seem original to you? & 
0 The title is very predictable, a pure cliché. \\
& & 1 The title is quite predictable and resorts to clichés. \\
& & 2 The title is quite original and avoids clichés. \\
& & 3 The title is unique and surprising, unlike anything you have seen before. \\
\hline
\textbf{Style} & Is the text's style original and surprising? & 
0 The style is formulaic and completely conventional. \\
& & 1 The style has some original elements but is predominantly conventional. \\
& & 2 The style is relatively original and is not easily comparable to other writers. \\
& & 3 The style is very original and reveals a unique voice of the writer. \\
\hline
\textbf{Plot} & Is the plot of the text original and introduces innovative elements? & 
0 The plot is completely conventional and relies on widely explored ideas or clichés without bringing new elements. \\
& & 1 The plot is quite conventional, although there are marginal attempts to introduce original elements. \\
& & 2 The plot is quite original and brings innovative elements. \\
& & 3 The plot is very original and innovative. \\
\hline
\end{longtable}

\section*{3. Considering that the title was the starting point of the literary exercise, do you think the writer has used it well?}

\begin{longtable}{|p{0.7\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Considering that the title was the starting point of the literary exercise, do you think the writer has used it well? & 
No relation at all between the title and the synopsis. \\
& The relation between the title and the synopsis is almost irrelevant. \\
& There is some relation between the title and the synopsis, although not evident. \\
& There is a lot of relation between the title and the synopsis, and the text's development is predictable from the title. \\
& There is a lot of relation between the title and the synopsis, and the connection is surprising; the way of developing the title is original. \\
\hline
\end{longtable}

\section*{4. Rate the creativity of:}

\begin{longtable}{|p{0.2\textwidth}|p{0.8\textwidth}|}
\hline
\textbf{Aspect} & \textbf{Options} \\
\hline
\textbf{Title} & 0 Not creative at all. \\
& 1 Slightly creative. \\
& 2 Quite creative. \\
& 3 Very creative. \\
\hline
\textbf{Synopsis} & 0 Not creative at all. \\
& 1 Slightly creative. \\
& 2 Quite creative. \\
& 3 Very creative. \\
\hline
\end{longtable}

\section*{5. Rate the authorship:}

\begin{longtable}{|p{0.7\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Who do you think wrote this title? & A novice writer. \\
& An established writer. \\
& An artificial intelligence. \\
\hline
Who do you think wrote the synopsis? & A novice writer. \\
& An established writer. \\
& An artificial intelligence. \\
\hline
\end{longtable}

\section*{6. The exercise of inventing a synopsis for an imaginary movie can be seen as a sort of literary genre. Imagine that this genre exists:}

\begin{longtable}{|p{0.7\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Question} & \textbf{Options} \\
\hline
Do you think you would select this text for an anthology of this genre? & 
0 Under no circumstances. \\
& 1 It is unlikely. \\
& 2 It is probable. \\
& 3 With certainty. \\
\hline
Do you think your evaluation of the text would align with the majority of readers? & 
0 Under no circumstances. \\
& 1 It is unlikely. \\
& 2 It is probable. \\
& 3 With certainty. \\
\hline
Do you think your evaluation of the text would align with the majority of literary critics? & 
0 Under no circumstances. \\
& 1 It is unlikely. \\
& 2 It is probable. \\
& 3 With certainty. \\
\hline
Judging only by this text, do you think it is likely that the author has a recognizable style, that is, a unique voice? & 
0 Under no circumstances. \\
& 1 It is unlikely. \\
& 2 It is probable. \\
& 3 With certainty. \\
\hline
\end{longtable}


